VideoGigaGAN: Towards Detail-rich Video Super-Resolution

Video super-resolution (VSR) approaches have shown impressive temporal consistency in upsampled videos. However, these approaches tend to generate blurrier results than their image counterparts as they are limited in their generative capability. This raises a fundamental question: can we extend the success of a generative image upsampler to the VSR task while preserving the temporal consistency? We introduce VideoGigaGAN, a new generative VSR model that can produce videos with high-frequency details and temporal consistency. VideoGigaGAN builds upon a large-scale image upsampler -- GigaGAN. Simply inflating GigaGAN to a video model by adding temporal modules produces severe temporal flickering. We identify several key issues and propose techniques that significantly improve the temporal consistency of upsampled videos. Our experiments show that, unlike previous VSR methods, VideoGigaGAN generates temporally consistent videos with more fine-grained appearance details. We validate the effectiveness of VideoGigaGAN by comparing it with state-of-the-art VSR models on public datasets and showcasing video results with $8\times$ super-resolution.

==> figures/quality_vs_temp_old.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{images/temp_vs_fidelity_tradeoff.pdf}
    \caption{Trade-off between per-frame quality (LPIPS) and temporal consistency (warping error).}
    \label{fig:tradeoff}
\end{figure}

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

% topic
\newcommand{\topic}[1]
{
\vspace{1mm}\noindent\textbf{#1}
}

% for math equations
\DeclareMathOperator*{\argmin}{\arg\!\min} 
\DeclareMathOperator*{\argmax}{\arg\!\max}
\DeclareMathOperator*{\minimize}{minimize}

% for tables
\usepackage{soul} % \ul
\usepackage{multirow}
\let\Bbbk\relax
\usepackage{amsmath, amssymb}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\usepackage{enumitem, array}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

\usepackage{blindtext}% for dummy text only
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
% Redefine subcaption label format
\DeclareCaptionSubType*[arabic]{figure}
\captionsetup[subfigure]{labelformat=empty}

% vertical rule
\newcommand{\rulesep}{\unskip\ \vrule\ }

% footnote
\usepackage[symbol]{footmisc}


==> tables/temp_comp.tex <==
\begin{table}[t!]
  \centering
  \caption{Comparison on temporal consistency v.s. per-frame fidelity.}
    \scriptsize
    \begin{tabular}{lrrr}
    \toprule
    Model & \multicolumn{1}{l}{LPIPS$\downarrow$} & \multicolumn{1}{l}{$E_{warp} \downarrow (\times 10^{-3})$ } & \multicolumn{1}{l}{$E^{ref}_{warp} \downarrow (\times 10^{-3})$ }\\
    \midrule
    EDVR~\cite{wang2019edvr} &  0.2097     &  1.521 & 2.1429\\
    MuCAN~\cite{li2020mucan} &   0.2162   &   1.562 & 2.1574\\
    BasicVSR~\cite{chan2021basicvsr} & 0.2023      &  1.371 & 2.1220\\
    IconVSR~\cite{chan2021basicvsr} &   0.1939    &  1.379 & 2.2119 \\
    TTVSR~\cite{liu2022learning}  &  0.1836     &  1.390 & 2.1178\\
    BasicVSR++~\cite{chan2022basicvsrpp} & 0.1786 &  1.401 & 2.1206\\
    Ours &   0.1582  &  2.313 & 2.1773\\
    \midrule
    GT   &   -  &  2.127 & - \\
    \bottomrule
    \end{tabular}%
  \label{tab:temp_comparison}%
\end{table}%

